Generalized Optimal Linear Orders

The sequential structure of language, and the order of words in a sentence specifically, plays a central role in human language processing. Consequently, in designing computational models of language, the de facto approach is to present sentences to machines with the words ordered in the same order as in the original human-authored sentence. The very essence of this work is to question the implicit assumption that this is desirable and inject theoretical soundness into the consideration of word order in natural language processing. In this thesis, we begin by uniting the disparate treatments of word order in cognitive science, psycholinguistics, computational linguistics, and natural language processing under a flexible algorithmic framework. We proceed to use this heterogeneous theoretical foundation as the basis for exploring new word orders with an undercurrent of psycholinguistic optimality. In particular, we focus on notions of dependency length minimization given the difficulties in human and computational language processing in handling long-distance dependencies. We then discuss algorithms for finding optimal word orders efficiently in spite of the combinatorial space of possibilities. We conclude by addressing the implications of these word orders on human language and their downstream impacts when integrated in computational models.

==> README <==
cornell-thesis 2.9
------------------

This package provides a "style file" for producing Ph.D. dissertations
at Cornell University using the new version of LaTeX, LaTeX 2e
which is now the only officially supported one. (If you haven't
upgraded to it yet, this file won't be of much use to you. Consider
upgrading.)

The distribution contains two source files:
cornell.dtx -- self-documenting LaTeX source code for the style file.
cornell.ins -- installation "script" for the docstrip package.

To install, you need to say "latex cornell.ins", then move the resulting
cornell.cls file somewhere where latex will find it.

Detailed (albeit still incomplete in places) documentation can be be
found in the file "cornell.pdf". This documentation can also be generated
by saying "pdflatex cornell.dtx" twice (or use latex if you want a .dvi file).

There is also a sample thesis document that you can use as a template
for writing your thesis, in "sampleThesis.tex". You can build this by
running "latex sampleThesis" and "bibtex sampleThesis" until things
converge (usually this takes three runs of "latex").

If you don't like typing "latex" so much, and you have "make" available,
you can type "make" to build the document class file and the sample
thesis document. You may also want to use the supplied Makefile as a starting
point for building your own thesis.

Comments from Sergio:

    This style file does not have official status: I just happen to have
    typeset my thesis with the new LateX 2e, using this style file, and the
    thesis secretary seemed fairly pleased with the result. I am making it
    available in the hope that the horror stories about people's encounters
    with the thesis secretary may become a thing of the past... but remember:
    requirements do change, and this style file doesn't remove the need for you
    to heed TeX's warning messages about overfull boxes and pages.

    An older style file for LaTeX 2.09 is still available in various places on
    campus. I used it as a starting point, but added a few enhancements of my
    own.

    I have no plans to maintain this thing. Users are on their own.  But at
    least I tried to document it as fully as time allowed me.

Change Log

v1.0d Converted ## to # as per changes in June 1995 LaTeX release.
v1.1  Changed openbib conditionals to a single command as per changes
           in December 1995 LaTeX release.
v1.2  Moved headers for opening pages to top of page.
v2.0  Chapter headers now consistent throughout.
      Fixed margins.
v2.1  Bug fix for titles containing \\
v2.5  Addition of halfcornellheadings and smallerheadings options
v2.6  Addition of draft, semifinal and final options
v2.7  Corrected interline spacing to really be double spacing
      (i.e, 24pt for 12pt text).  Changed ``cornell'' pagestyle to
      center page numbers at the bottom of the page.
v2.8  When using pdflatex, page size is set to 8.5x11 automatically.
      Copyright and dedication now center properly on page without special hacks.
      \ifpdf macro added to detect use of pdflatex
      A sample thesis document is included in the package.
      A sample Makefile is included in the package (use is optional).
v2.9  Made "cornellheadings" the default, as the thesis guidelines now
      require them for appendices. Also fixed line spacing and margins
      on the title page. Changed sample document to palatino, since
      Times 12 is not approved.


==> commondefs <==
#
# Rules and definitions for building various things, especially 
# TeX documents.
# -- Andrew Myers
# Last updated April 2007
#

MAKEDIR = .
INCLDIR = .
TEXDIR = .

COMMONRULES = $(MAKEDIR)/commonrules

SOURCES = $(CFILES) $(C++FILES) $(YFILES) $(LFILES) $(AFILES)
OBJECTS = $(CFILES:.c=.o) $(C++FILES:.C=.o)
DIRT = *.o core *.aux *.dvi *.log *.stamp *.i *.bbl *.[ib]lg $(LDIRT)
GENERATED = .dependtime Makedepend Makedepend.bak
RM = rm -f
MKDEPFILE = Makedepend
MKDEPEND = makedepend
MKDEPFLAGS = -Y
MKDEPC++FLAGS = $(C++DEFS) $(C++INCS) $(MKDEPFLAGS)
MKDEPCFLAGS = $(CDEFS) $(CINCS) $(MKDEPFLAGS)

.SUFFIXES: .C .ps .i .txt .h
.SUFFIXES: .tex .dvi .ind .idx .bbl .aux .glo .aux .stamp .pdf .eps

GNUBIN = /usr/local

ATTC++ = CC
DECC++ = cxx
GNUC++ = g++

CC = cc
C++ = $(GNUC++)
YACC = bison
DVIPS = dvips

C++F = $(C++) $(C++FLAGS)
CCF = $(CC) $(CFLAGS)

C++FLAGS = $(C++OPTS) $(C++DEFS) $(C++INCS)

C++INCS = $(GC++INCS) $(LC++INCS)
C++OPTS = $(GC++OPTS) $(LC++OPTS)
C++DEFS = $(GC++DEFS) $(LC++DEFS)

GC++OPTS = $(OPTIMIZER)

CFLAGS = $(COPTS) $(CDEFS) $(CINCS)
COPTS = $(GCOPTS) $(LCOPTS)
CDEFS = $(GCDEFS) $(LCDEFS)
CINCS = $(GCINCS) $(LCINCS)

GCOPTS = $(OPTIMIZER)

M3F = $(M3) $(M3FLAGS)
M3 = m3
M3PP = m3pp

LDFLAGS = $(LLDFLAGS) $(GLDFLAGS)
LLDFLAGS = $(LLDLIBS) $(LLDOPTS) 

SEP=:
#SEP=\;         # for MikTeX+Cygwin
TEXINPUTS = .$(SEP)$(TEXDIR)$(SEP)
LATEX = TEXINPUTS=$(TEXINPUTS) latex
PDFLATEX = TEXINPUTS=$(TEXINPUTS) pdflatex


==> commonrules <==
# Some basic recursive rules for building, installing, and cleaning up
# a source tree
#
subdirs:
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make); \
	fi; done;

clean:  localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

localclean:
	$(RM) $(DIRT)

clobber: localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;
	$(RM) $(TARGETS) $(GENERATED)

install: default localinstall
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

incdepend: .dependtime
depend: .dependtime

.dependtime: $(SOURCES)
	touch temp
	$(MKDEPEND) $(MKDEPC++FLAGS) -f temp $(C++FILES)
	touch $(MKDEPFILE)
	$(MKDEPEND) $(MKDEPCFLAGS) -f $(MKDEPFILE) $(CFILES)
	cat temp >> $(MKDEPFILE)
	rm -f temp
	touch $@

# Rules for TeX files
#
# The line that runs LATEX needs to run inside a subshell to turn off
# "make"'s status checking. It blows away .aux because the .aux file
# created is bad and also breaks bibtex. It touches .stamp to force a
# rebuild.
.tex.dvi:
	@if test -r "$*.aux"; \
	   then cp $*.aux $*.auxprev; \
	   else echo > $*.auxprev; \
	fi
	@echo "$(LATEX) $<"
	@sh -c "$(LATEX) $< || (rm -f $*.aux; sleep 1; touch $*.stamp; exit 1)"
	@-cmp -s $*.aux $*.auxprev; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch $*.stamp; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f $*.auxprev

.tex.pdf:
	@if test -r "$*.aux"; \
	   then cp $*.aux $*.auxprev; \
	   else echo > $*.auxprev; \
	fi
	@echo "$(PDFLATEX) $<"
	@sh -c "$(PDFLATEX) $< || (rm -f $*.aux; sleep 1; touch $*.stamp; exit 1)"
	@-cmp -s $*.aux $*.auxprev; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch $*.stamp; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f $*.auxprev

# must add dependencies like
#    foo.ind: foo.stamp
#    foo.dvi: foo.ind
# to use this rule properly.
.tex.ind:
	@if [ -f $*.idx ]; then \
	   echo makeindex $*.idx; \
	   makeindex $*.idx; \
	else \
	   echo touch $@; \
	   touch $@; \
        fi

# must add dependencies like
#    foo.bbl: foo.bib
#    foo.dvi: foo.bbl
# to use this rule properly.
.tex.bbl:
	@if [ -r $*.aux ]; then echo bibtex $*; sh -c "bibtex $(BIBOPTS) $* || echo"; else echo; fi

.tex.stamp: # backward compatibility
	touch $@

.dvi.ps:
	$(DVIPS) $(DVIPSOPTS) $< -o $@
.eps.pdf:
	epstopdf $<

#
# Rules for C++ and .i files
#

.C.i:
	$(C++F) -E $< > $@

.c.i:
	$(CCF) -E $< > $@

.C.o:
	$(C++F) -c $<

# include $(M3SU)    # old Modula-3 rules


==> tables/additional_results/pool=max-p=0.0-h=32.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.847 & 0.952 & 0.874 & 0.477 & 0.95 \\
$r_r$ & 0.841 & 0.947 & 0.871 & 0.473 & 0.944 \\
\midrule
$r_b$ & 0.844 & 0.945 & 0.87 & 0.476 & 0.962 \\
$r_c$ & 0.852 & 0.95 & 0.873 & 0.482 & 0.952 \\
$r_m$ & 0.841 & 0.946 & 0.866 & 0.495 & 0.958 \\
\midrule
$\tilde{r}_b$ & 0.839 & 0.953 & 0.881 & 0.488 & 0.954 \\
$\tilde{r}_c$ & 0.833 & 0.952 & 0.877 & 0.495 & 0.954 \\
$\tilde{r}_m$ & 0.844 & 0.958 & 0.877 & 0.49 & 0.954 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 32, p = 0.0$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.0-h=32}
\end{table*}


==> tables/additional_results/pool=max-p=0.02-h=128.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.86 & 0.951 & 0.885 & 0.49 & 0.966 \\
$r_r$ & 0.847 & 0.95 & 0.881 & 0.498 & 0.952 \\
\midrule
$r_b$ & 0.844 & 0.951 & 0.88 & 0.486 & 0.958 \\
$r_c$ & 0.862 & 0.953 & 0.874 & 0.491 & 0.96 \\
$r_m$ & 0.844 & 0.952 & 0.876 & 0.482 & 0.97 \\
\midrule
$\tilde{r}_b$ & 0.86 & 0.949 & 0.882 & 0.486 & 0.954 \\
$\tilde{r}_c$ & 0.852 & 0.953 & 0.873 & 0.494 & 0.966 \\
$\tilde{r}_m$ & 0.839 & 0.952 & 0.885 & 0.487 & 0.962 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 128, p = 0.02$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.02-h=128}
\end{table*}


==> tables/additional_results/pool=max-p=0.02-h=64.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.839 & 0.955 & 0.882 & 0.495 & 0.96 \\
$r_r$ & 0.844 & 0.949 & 0.874 & 0.486 & 0.954 \\
\midrule
$r_b$ & 0.854 & 0.95 & 0.871 & 0.5 & 0.96 \\
$r_c$ & 0.836 & 0.946 & 0.874 & 0.478 & 0.96 \\
$r_m$ & 0.836 & 0.951 & 0.877 & 0.473 & 0.964 \\
\midrule
$\tilde{r}_b$ & 0.847 & 0.948 & 0.878 & 0.472 & 0.96 \\
$\tilde{r}_c$ & 0.852 & 0.956 & 0.873 & 0.499 & 0.958 \\
$\tilde{r}_m$ & 0.833 & 0.953 & 0.875 & 0.486 & 0.964 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 64, p = 0.02$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.02-h=64}
\end{table*}


==> tables/additional_results/pool=max-p=0.2-h=128.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.847 & 0.948 & 0.874 & 0.491 & 0.96 \\
$r_r$ & 0.852 & 0.952 & 0.87 & 0.496 & 0.952 \\
\midrule
$r_b$ & 0.833 & 0.955 & 0.873 & 0.5 & 0.954 \\
$r_c$ & 0.857 & 0.946 & 0.879 & 0.482 & 0.964 \\
$r_m$ & 0.828 & 0.947 & 0.875 & 0.494 & 0.962 \\
\midrule
$\tilde{r}_b$ & 0.847 & 0.943 & 0.874 & 0.49 & 0.95 \\
$\tilde{r}_c$ & 0.854 & 0.953 & 0.882 & 0.483 & 0.956 \\
$\tilde{r}_m$ & 0.847 & 0.951 & 0.874 & 0.491 & 0.958 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 128, p = 0.2$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.2-h=128}
\end{table*}


==> tables/additional_results/pool=max-p=0.2-h=256.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.862 & 0.957 & 0.896 & 0.502 & 0.968 \\
$r_r$ & 0.862 & 0.949 & 0.877 & 0.482 & 0.968 \\
\midrule
$r_b$ & 0.849 & 0.957 & 0.873 & 0.488 & 0.966 \\
$r_c$ & 0.854 & 0.947 & 0.871 & 0.475 & 0.958 \\
$r_m$ & 0.847 & 0.953 & 0.878 & 0.491 & 0.96 \\
\midrule
$\tilde{r}_b$ & 0.854 & 0.952 & 0.88 & 0.482 & 0.96 \\
$\tilde{r}_c$ & 0.852 & 0.947 & 0.875 & 0.499 & 0.968 \\
$\tilde{r}_m$ & 0.841 & 0.948 & 0.871 & 0.485 & 0.964 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 256, p = 0.2$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.2-h=256}
\end{table*}


==> tables/additional_results/pool=max-p=0.2-h=64.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.833 & 0.954 & 0.878 & 0.496 & 0.96 \\
$r_r$ & 0.831 & 0.945 & 0.876 & 0.493 & 0.956 \\
\midrule
$r_b$ & 0.849 & 0.949 & 0.87 & 0.49 & 0.962 \\
$r_c$ & 0.852 & 0.951 & 0.871 & 0.49 & 0.964 \\
$r_m$ & 0.839 & 0.947 & 0.878 & 0.484 & 0.96 \\
\midrule
$\tilde{r}_b$ & 0.852 & 0.949 & 0.87 & 0.481 & 0.958 \\
$\tilde{r}_c$ & 0.854 & 0.957 & 0.874 & 0.49 & 0.952 \\
$\tilde{r}_m$ & 0.839 & 0.956 & 0.884 & 0.501 & 0.97 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 64, p = 0.2$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.2-h=64}
\end{table*}


==> tables/additional_results/pool=mean-p=0.0-h=32.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.841 & 0.948 & 0.871 & 0.466 & 0.947 \\
$r_r$ & 0.829 & 0.942 & 0.867 & 0.453 & 0.942 \\
\midrule
$r_b$ & 0.842 & 0.942 & 0.868 & 0.459 & 0.951 \\
$r_c$ & 0.838 & 0.948 & 0.871 & 0.462 & 0.947 \\
$r_m$ & 0.835 & 0.944 & 0.862 & 0.473 & 0.951 \\
\midrule
$\tilde{r}_b$ & 0.832 & 0.946 & 0.877 & 0.472 & 0.951 \\
$\tilde{r}_c$ & 0.828 & 0.95 & 0.873 & 0.474 & 0.95 \\
$\tilde{r}_m$ & 0.837 & 0.952 & 0.875 & 0.461 & 0.949 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 32, p = 0.0$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.0-h=32}
\end{table*}


==> tables/additional_results/pool=mean-p=0.02-h=128.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.844 & 0.951 & 0.881 & 0.485 & 0.957 \\
$r_r$ & 0.842 & 0.947 & 0.876 & 0.477 & 0.948 \\
\midrule
$r_b$ & 0.837 & 0.949 & 0.875 & 0.474 & 0.952 \\
$r_c$ & 0.845 & 0.947 & 0.872 & 0.48 & 0.954 \\
$r_m$ & 0.833 & 0.951 & 0.872 & 0.471 & 0.952 \\
\midrule
$\tilde{r}_b$ & 0.85 & 0.947 & 0.878 & 0.468 & 0.95 \\
$\tilde{r}_c$ & 0.848 & 0.951 & 0.867 & 0.484 & 0.962 \\
$\tilde{r}_m$ & 0.834 & 0.95 & 0.878 & 0.469 & 0.957 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 128, p = 0.02$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.02-h=128}
\end{table*}


==> tables/additional_results/pool=mean-p=0.02-h=64.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.832 & 0.952 & 0.876 & 0.468 & 0.956 \\
$r_r$ & 0.833 & 0.946 & 0.865 & 0.467 & 0.949 \\
\midrule
$r_b$ & 0.85 & 0.946 & 0.866 & 0.475 & 0.958 \\
$r_c$ & 0.827 & 0.942 & 0.872 & 0.473 & 0.95 \\
$r_m$ & 0.829 & 0.949 & 0.868 & 0.461 & 0.956 \\
\midrule
$\tilde{r}_b$ & 0.842 & 0.944 & 0.868 & 0.466 & 0.954 \\
$\tilde{r}_c$ & 0.844 & 0.952 & 0.867 & 0.47 & 0.957 \\
$\tilde{r}_m$ & 0.826 & 0.948 & 0.869 & 0.465 & 0.958 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 64, p = 0.02$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.02-h=64}
\end{table*}


==> tables/additional_results/pool=mean-p=0.2-h=128.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.835 & 0.945 & 0.866 & 0.476 & 0.954 \\
$r_r$ & 0.842 & 0.944 & 0.865 & 0.45 & 0.95 \\
\midrule
$r_b$ & 0.83 & 0.948 & 0.866 & 0.473 & 0.951 \\
$r_c$ & 0.854 & 0.938 & 0.869 & 0.471 & 0.957 \\
$r_m$ & 0.817 & 0.941 & 0.865 & 0.463 & 0.955 \\
\midrule
$\tilde{r}_b$ & 0.828 & 0.941 & 0.868 & 0.477 & 0.947 \\
$\tilde{r}_c$ & 0.848 & 0.947 & 0.87 & 0.471 & 0.953 \\
$\tilde{r}_m$ & 0.843 & 0.943 & 0.865 & 0.471 & 0.951 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 128, p = 0.2$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.2-h=128}
\end{table*}


==> tables/additional_results/pool=mean-p=0.2-h=256.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.843 & 0.952 & 0.885 & 0.483 & 0.96 \\
$r_r$ & 0.845 & 0.943 & 0.871 & 0.464 & 0.951 \\
\midrule
$r_b$ & 0.828 & 0.951 & 0.863 & 0.465 & 0.958 \\
$r_c$ & 0.841 & 0.941 & 0.863 & 0.469 & 0.955 \\
$r_m$ & 0.822 & 0.945 & 0.865 & 0.479 & 0.957 \\
\midrule
$\tilde{r}_b$ & 0.847 & 0.948 & 0.866 & 0.468 & 0.957 \\
$\tilde{r}_c$ & 0.828 & 0.943 & 0.87 & 0.482 & 0.959 \\
$\tilde{r}_m$ & 0.838 & 0.944 & 0.866 & 0.476 & 0.958 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 256, p = 0.2$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.2-h=256}
\end{table*}


==> tables/additional_results/pool=mean-p=0.2-h=64.table.tex <==
\begin{table*}[t]
\centering
\large{
\begin{tabular}{cccccc}
\toprule
& \texttt{CR} & \texttt{SUBJ} & \texttt{SST-2} & \texttt{SST-5} & \texttt{TREC} \\
\midrule
$r_I$ & 0.815 & 0.952 & 0.875 & 0.481 & 0.956 \\
$r_r$ & 0.824 & 0.942 & 0.868 & 0.464 & 0.952 \\
\midrule
$r_b$ & 0.829 & 0.945 & 0.864 & 0.475 & 0.956 \\
$r_c$ & 0.841 & 0.947 & 0.867 & 0.478 & 0.953 \\
$r_m$ & 0.832 & 0.936 & 0.869 & 0.468 & 0.951 \\
\midrule
$\tilde{r}_b$ & 0.847 & 0.946 & 0.864 & 0.477 & 0.954 \\
$\tilde{r}_c$ & 0.838 & 0.948 & 0.867 & 0.482 & 0.945 \\
$\tilde{r}_m$ & 0.825 & 0.948 & 0.873 & 0.475 & 0.956 \\
\bottomrule
\end{tabular}}
\caption{Classification Results for $h = 64, p = 0.2$. Results use \texttt{pretrain-permute-finetune} framework with the order specified in each row. All other hyperparameters are set as described previously. The top part of the table refers to baselines. The middle part of the table refers to orders derived from pure optimization algorithms. The bottom part of the table refers to orders derived from heuristic algorithms we introduce using \texttt{Transposition Monte Carlo}. }
\label{tab:p=0.2-h=64}
\end{table*}

